Magnetic domain wall substructures in Pt/Co/Ni/Ir multi-layers

We examine the substructures of magnetic domain walls (DWs) in [Pt/(Co/Ni)$_M$/Ir]$_N$ multi-layers using a combination of micromagnetic theory and Lorentz transmission electron microscopy (LTEM). Thermal stability calculations of Q=$\pm$1 substructures (2-$\pi$ vertical Bloch lines (VBLs) and DW skyrmions) were performed using a geodesic nudged elastic band (GNEB) model, which supports their metastability at room temperature. Experimental variation in strength of the interfacial Dzyaloshinskii-Moriya interaction (DMI) and film thickness reveals conditions under which these substructures are present and enables the formation of a magnetic phase diagram. Reduced thickness is found to favor Q=$\pm$1 substructures likely due to the suppression of hybrid DWs. The results from this study provide an important framework for examining 1-D DW substructures in chiral magnetic materials.

==> DW skyrmions JAP arxiv/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
